Joint Visual Semantic Reasoning: Multi-Stage Decoder for Text Recognition

Although text recognition has significantly evolved over the years, state-of-the-art (SOTA) models still struggle in the wild scenarios due to complex backgrounds, varying fonts, uncontrolled illuminations, distortions and other artefacts. This is because such models solely depend on visual information for text recognition, thus lacking semantic reasoning capabilities. In this paper, we argue that semantic information offers a complementary role in addition to visual only. More specifically, we additionally utilize semantic information by proposing a multi-stage multi-scale attentional decoder that performs joint visual-semantic reasoning. Our novelty lies in the intuition that for text recognition, the prediction should be refined in a stage-wise manner. Therefore our key contribution is in designing a stage-wise unrolling attentional decoder where non-differentiability, invoked by discretely predicted character labels, needs to be bypassed for end-to-end training. While the first stage predicts using visual features, subsequent stages refine on top of it using joint visual-semantic information. Additionally, we introduce multi-scale 2D attention along with dense and residual connections between different stages to deal with varying scales of character sizes, for better performance and faster convergence during training. Experimental results show our approach to outperform existing SOTA methods by a considerable margin.

==> arguments.tex <==
Our proposed model gets 84\% accuracy on IC15 which is an improvement of 9.5\% over 74.5\%.

# L464 Using teacher-forcing on each stage does not give any performance boost but rather decreases performance by 0.1\% from 74.5\%. Argument: Since the refining process is not learnt, those additional decoders only make the model more complex without learning any new knowledge. Hence, performance dips slightly.

# L671 Using straight-through estimators creates instability which reduces model performance from 84.0\% to 82.8\%, a drop of 3.9\%

# Replacing Embedding network E(\cdot) with a FC-layer drops performance by 1.2\% i.e. goes from 84.0\% to 82.8\%

# Use reverse of top-down for attentional decoder i.e. $B_{L-2}$, $B_{L-1}$ ..., drops performance to 72.1\% i.e. a drop of 2.4\% from original IC15 74.5\%

# Removing visual reasoning drop by 2.9\% and removing semantic reasoning drops by 4.8\% and removing both drops 6.9\% from our final performance of 84.0\%.

# Instead of multi-scale feature if used $B_{L}$ for all stages performance drops to 81.3\% a drop of 2.7\%

# Using Pyramid Pooling instead of Feature Pyramid Networks drop performance by 2.1\% to 81.9\%

# Removing dense connection reduces performance by 1.6\%, removing residual connections drops by 1.3\% and removing both drops by 1.9\%

# Imposing $L_{C}$ only in the last stage fails and drops to 73.1\% and multi-stage $L_{C}$ gives 77.1\%

# Transformer for joint visual-semantic outperforms LSTM by 1.3\%

# All weight sharing drops to 82.3\% and all distict weight gives 82.5\%. Selective sharing gives 84.0\%

==> pinaki-backup.tex <==
\begin{table*}
\centering
\caption{Comparison of the proposed method with existing text recognition techniques in the past few years.}
\resizebox{2.\columnwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|l}
\hline\hline
\textbf{Methods} & \textbf{Year}  & \textbf{IIIT-5K} & \textbf{SVT} & \textbf{IC13} & \textbf{IC15} & \textbf{SVT-P} & \textbf{CUTE80} & \textbf{Remarks} \\
\hline
    Shi \etal \cite{Shi2015} & 2015 & 81.2 & 82.7 & 89.6 & - & 66.8 & 54.9 & End-to-end trainable CNN + RNN + CTC framework \\
    \hline
    Lee and Osindero \cite{lee2016recursive} & 2016 & 78.4 & 80.7 & - & 90.8 & - & 42.7 & Recursive CNN + RNN for LM + Soft Atten. decoder \\
    Shi \etal \cite{shi2016rare} & 2016 & 81.9 & 81.9 & 88.6 & - & - & - & Spatial Transformer Network(STN) + CNN + RNN + Atten. decoder \\
    \hline
    Cheng \etal \cite{cheng2017focusing} & 2017 & 87.4 & 85.9 & 93.3 & 70.6 & 71.5 & 63.9 & Char. annot. + Atten. drift + CNN-RNN-Atten. decoder \\
    \hline
    Liu \etal \cite{liu2018charnet} & 2018 & 83.6 & 84.4 & - & 60.0 & 73.5 & - & Char. annot. + CNN + Hierarchial Atten. Mechanism + LSTM-decoder \\
    Bai \etal \cite{bai2018edit} & 2018 & 88.3 & 87.5 & 94.4 & 73.9 & - & - & Char. annot. + CNN + RNN + Edit Prob. based Atten. decoder \\
    Liu \etal \cite{liu2018feature} & 2018 & 89.4 & 87.1 & 94.0 & - & 73.9 & 62.5 & Char. annot. + CNN + bLSTM + CTC + GAN \\
    Shi \etal \cite{shi2018aster} & 2018 & 93.4 & 93.6 & 91.8 & 76.1 & 78.5 & 79.5 & Thin Plate Spline(TPS) Img. rectification + CNN-RNN-Atten. decoder \\
    Cheng \etal \cite{cheng2018aon} & 2018 & 87.0 & 82.8 & - & 68.2 & 73.0 & 76.8 & CNN + 4 directional Atten. + bLSTM + Atten. decoder \\
    \hline
    Liao \etal \cite{liao2019scene} & 2019 & 91.9 & 86.4 & 91.5 & - & - & 79.9 & Char. Atten. FCN with pixel classification in 2D fashion \\
    % Liao \etal \cite{liao2019maskTextspotter} & 2019 & 95.3 & 91.8 & 95.3 & 78.2 & 83.6 & 88.5 \\
    Yang \etal \cite{yang2019symmetry} & 2019 & 94.4 & 88.9 & 93.9 & 78.7 & 80.8 & 87.5 & Geometrical attributes + TPS for rectification + CNN-RNN-Atten. decoder \\L a ahttps://tse1.mm.bing.net/th?id=OGC.cdc87c1875156c86c127410f7cc0ff0d&pid=Api&rurl=https%3a%2f%2fmedia.giphy.com%2fmedia%2fuADXDOFGgcVXO%2fgiphy.gif&ehk=LxeTJmXCSMPTD4I1WMB8Q0RSQRgQHOSG3Vic27T0GuI%3d 
    Luo \etal \cite{moran} & 2019 & 91.2 & 88.3 & 92.4 & 68.8 & 76.1 & 77.4 & Geometric constraints Free STN + CNN + bLSTM + Fractional Pickup + Atten. decoder \\
    Li \etal \cite{li2019show} & 2019 & 95.0 & 91.2 & 94.0 & 78.8 & 86.4 & 89.6 & CNN + bLSTM + 2D Atten. decoder\\
    Baek \etal \cite{baek2019wrong} & 2019 & 87.9 & 87.5 & 92.3 & 71.8 & 79.2 & 74.0 & holistic \& fair comparison of STR method; 4-stage generalised framework for STR \\
    Zhan \etal \cite{ESIR2019} & 2019 & 93.3 & 90.2 & 91.3 & 76.9 & 79.6 & 83.3 & Iterative Image rectification + CNN-RNN-Atten. decoder \\
    \hline
    Litman \etal \cite{litman2020scatter} & 2020 & 93.7 & 92.7 & 93.9 & 82.2 & 86.9 & 87.5 & Img. rectification + CNN + bLSTM + Visual Feature Refine + Selective-Decoder \\
    Qiao \etal \cite{qiao2020seed} & 2020 & 93.8 & 89.6 & 92.8 & 80.0 & 81.4 & 83.6 & Img. rectification + CNN + bLSTM + Global Semantic info. from LM + Atten. decoder \\
    Yu \etal \cite{yu2020towards} & 2020 & 94.8 & 91.5 & 95.5 & 82.7 & 85.1 & 87.8 & CNN+Parallel Visual Atten.+Global Semantic Reasoning+Visual-Semantic Fusion Decoder \\
    \hline
    Proposed Method & 2021 & xxx & xxx & xxx & xxx & xxx & xxx \\
    \hline
\end{tabular}}
\end{table*}

==> trash.tex <==
% \begin{table}[htb]%\[!htb\]
%     \caption{Global caption}
%     \begin{subtable}[t]{.5\textwidth}
%         \caption{This is a very very very long Caption}
%         \raggedright
%             \begin{tabular}{@{\extracolsep{1pt}}lcccc}
%                 \hline\hline \\
%                 Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Max} \\
%                 \hline \\
%                 A & 1.000 & 0.000 & 1     & 1 \\
%                 B & 0.968 & 0.76  & 0.138 & 1.000 \\
%                 C & 0.969 & 0.009 & 0.917 & 1.000 \\
%                 D & 0.966 & 0.070 & 0.495 & 0.83 \\
%                 \hline \\
%             \end{tabular}
%     \end{subtable}%
%   \begin{subtable}[t]{.5\textwidth}
%         \raggedleft
%         \caption{This is a very very very long Caption}
%         \begin{tabular}{@{\extracolsep{1pt}}lcccc}
%             \hline\hline \\
%         Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Max} \\
%         \hline \\
%                 A & 2.000 & 0.000 & 1     & 1 \\
%                 B & 0.968 & 0.76  & 0.138 & 1.000 \\
%                 C & 0.969 & 0.009 & 0.917 & 1.000 \\
%                 D & 0.966 & 0.070 & 0.495 & 0.83 \\
%         \hline \\
%         \end{tabular}
%     \end{subtable}
% \end{table}


% \begin{minipage}{0.5in}
%     \begin{tabular}{ccc}
%         A & B & C \\
%         \hline
%         1 & 2 & 3 \\
%         \hline
%         C & B & A \\
%     \caption{hi there}
%     \end{tabular}
% \end{minipage}
% \begin{minipage}{0.5in}
%     \begin{tabular}{ccc}
%         D & E & F \\
%         \hline
%         4 & 5 & 6 \\
%         \hline
%         F & E & D \\
%     \end{tabular}    
% \end{minipage}

% \begin{table}[!ht]
%     \caption{Results for testset0-1 (left) and testset0-2 (right)}
%     \begin{sideways}
%         \begin{minipage}[b]{0.25\linewidth}
%         \centering
%             \begin{tabular}{ccc}
%             % \caption{hi there}
%                 D & E & F \\
%                 \hline
%                 4 & 5 & 6 \\
%                 \hline
%                 F & E & D \\
%             \end{tabular}  
%         \end{minipage}
%     \end{sideways}
%     \begin{sideways}
%         \begin{minipage}[b]{0.25\linewidth}
%             \centering
%             \begin{tabular}{ccc}
%             % \caption{hi there2}
%                 D & E & F \\
%                 \hline
%                 4 & 5 & 6 \\
%                 \hline
%                 F & E & D \\
%             \end{tabular}    
%         \end{minipage}
%     \end{sideways}
% \end{table}
